LightLoc: Learning Outdoor LiDAR Localization at Light Speed

Scene coordinate regression achieves impressive results in outdoor LiDAR localization but requires days of training. Since training needs to be repeated for each new scene, long training times make these methods impractical for time-sensitive applications, such as autonomous driving, drones, and robotics. We identify large coverage areas and vast data in large-scale outdoor scenes as key challenges that limit fast training. In this paper, we propose LightLoc, the first method capable of efficiently learning localization in a new scene at light speed. LightLoc introduces two novel techniques to address these challenges. First, we introduce sample classification guidance to assist regression learning, reducing ambiguity from similar samples and improving training efficiency. Second, we propose redundant sample downsampling to remove well-learned frames during training, reducing training time without compromising accuracy. Additionally, the fast training and confidence estimation capabilities of sample classification enable its integration into SLAM, effectively eliminating error accumulation. Extensive experiments on large-scale outdoor datasets demonstrate that LightLoc achieves state-of-the-art performance with a 50x reduction in training time than existing methods. Our code is available at https://github.com/liw95/LightLoc.

==> alg2.tex <==
\begin{algorithm}[t]
	\caption{Pseudocode for RFD} %算法的名字
	{\bf Input:} %算法的输入， \hspace*{0.02in}用来控制位置，同时利用 \\ 进行换行
	Training $\cal T$, pruning ratio $r_p$, start ratio $r_{st}$, stop ratio $r_{sp}$, training epochs $K$, length of window $W$.\\
	{\bf Initialization:} %算法的初始化
	Compute first pruning epochs $K_1\gets\lceil K\times r_s\rceil$; Second pruning epochs $K_2\gets\lfloor K\times \frac{r_e+r_s}{2}\rfloor$; Stop pruning epochs $K_s \gets \lfloor K\times r_{sp} \rfloor$. $\cal T \gets \cal T^{'}$
	\begin{algorithmic}[1]
		\For {$k=0, \ldots, K-1$}
		\State $\triangleright$ In parallel on GPUs
		\State Sample a batch $\cal{B}\sim \cal{T}$. 
		\For{$({\cal P}_i,{\cal P}_i^{*}) \in \cal{B}$}
        \State Compute the median of $L_1$ loss as ${\cal L}_m$.
        \If{$k \in \left[ K_j, K_j+W\right)$}    \tcp $j\in\left[1,2\right]$
        \State Compute the variance $\cal V$ of ${\cal L}_m$ in W.
        \EndIf
        \EndFor
        \If{$k = K_j + W$}
        \State Sort ${\cal T}^{'}$ in descending order of $\cal V$.
        \State ${\cal T}^{'} \gets$ front $(1-r)\times\left|{\cal T}^{'}\right|$ samples.
        \EndIf
        \If{$k = K_s$}
        \State ${\cal T}^{'} \gets \cal T$.
        \EndIf
        \State \Return ${\cal T}^{'}$
		\EndFor
	\end{algorithmic}
	\label{alg:1}
\end{algorithm}

==> eq/sup_eq1.tex <==
\begin{equation}
F_{k_1}= h_{bs}\left(F\right), \quad F_{k_2} = h_{bs}\left(h_{hp}\left(F_{k_1}\right)\right),
\label{sup_eq1}
\end{equation}
